Scalable and interpretable product recommendations via overlapping co-clustering

We consider the problem of generating interpretable recommendations by identifying overlapping co-clusters of clients and products, based only on positive or implicit feedback. Our approach is applicable on very large datasets because it exhibits almost linear complexity in the input examples and the number of co-clusters. We show, both on real industrial data and on publicly available datasets, that the recommendation accuracy of our algorithm is competitive to that of state-of-art matrix factorization techniques. In addition, our technique has the advantage of offering recommendations that are textually and visually interpretable. Finally, we examine how to implement our technique efficiently on Graphical Processing Units (GPUs).

==> Overlapping CoClusters (2017)/B2CvsB2B.tex <==
\section{B2C vs B2C recommendations}

Our main application of interest, albeit by far not the only one, in the problem of generating interpretable recommendation from one-class examples are B2B recommender systems. 
A B2B recommender system---in contrast to a Business-to-Consumer (B2C) recommender system (referring to recommender systems employed at sites such as Amazon.com or the Genius recommendations of Apple within their iTunes platform)---is typically not open to the public, but is deployed within an enterprise. Because only a handful of literature is available on B2B recommender systems \cite{DBLP:conf/icwe/OpreaHZEL13,DBLP:conf/iat/ZieglerOHEL13, B2B_ecommerce},
 we briefly point out some differences between a B2C and B2B deployment.
This discussion will serve the purpose of highlighting the need for higher interpretability in a B2B recommendation environment. %The discussion will also help highlight the different assumptions in data availability for both systems. 
%\RH{Commented this out, as the problem really arises in both B2B as well as B2C environments..}

\begin{enumerate}

\item The \textbf{system users} in a B2C system are the consumers, whereas in B2B they are the selling teams or marketing teams of an enterprise. Therefore the recommendations have a different audience.

\item The \textbf{user entities} (``clients") for which the recommendations are created are typically individuals in a B2C setting. In B2B, they are enterprises or companies. This has certain implications on data availability. For example, in B2C we have knowledge about past buying patterns (PBP) or implied interest from items browsed by the users. In B2B, we know the past buying patterns and it is also possible to obtain other type of information about the clients-companies in the form of news events or financial reports published about that company. This eventually can help build a more holistic view of the examined bipartite graph of clients and products.

\item The \textbf{value of the recommendation} in a B2C setting is typically small, ranging from a few dollars (a song or a movie) to a few hundreds of dollars (an electronic gadget). In contrast, in a B2B setting, the recommendation may refer to a large hardware installation or complex and custom software solution and the recommendation may be valued at thousands of dollars, or even millions. It is also interesting to note that in B2C the value of a product/recommendation  is (mostly) fixed, or it is publicly available, whereas in B2B it varies based on the complexity of the installation.

\item Finally, the \textbf{reasoning} of the recommendation is short and limited in a B2C scenario, but it has to be detailed and offer sufficient supportive evidence in B2B. This is partially because of the associated value of the recommendation. If a salesperson is to pursue a multi-thousand dollar sales opportunity, the methodology has to present sufficient reasoning for this action, which is subsequently further evaluated by the responsible seller or marketing team.

\end{enumerate}

%These points are summarized in Table \ref{tab:differences}. 
In this work we will only focus on the last part, the reasoning of the recommendation. Even though components such as estimating the appropriate value of a B2B recommendation are also non-trivial, they will not be further examined in this work.

% \begin{table*}[]
%     \centering
%     \caption{Differences between a B2C and B2B recommender system}
%     \label{tab:differences}
%     \small
%   \centering
%  \resizebox{.98\columnwidth}{!}{%
%     \begin{tabular}{l l l}
%          & \textbf{B2C}  & \textbf{B2B} \\  \hline
%         \textbf{users of system} & consumers & sellers/marketing teams\\
%          \textbf{``clients"}       & consumers & enterprises/companies \\
%          \textbf{what we know about clients}            & past buying patterns (PBP) & PBP, news, financials,... \\
%          \textbf{value of recommendation} & small to medium &  medium to high \\
%          \textbf{reasoning of recommendation} & limited  & detailed \\ 
%     \end{tabular}
%     } %resizebox
% \end{table*}


In the following section we begin to describe our approach for generating interpretable recommendations based on the client-product purchase graph.





==> Overlapping CoClusters (2017)/extra_information.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\vspace{-2\baselineskip}
\section{Adding extra information}
\label{sec:incorpatt}

While the focus of this paper is on generating recommendations based on positive examples only, e.g., on the purchase history of clients, we explain briefly  how to incorporate additional information in the OCuLaR algorithm. 
This is important for addressing the cold-start problem, i.e., for making recommendations to users that have no purchase history, or for recommending items that have not been purchased. In addition, it can also improve the recommendation performance for users/items for which positive examples exist. 
%An astute reader would have noticed that the algorithm, as previously described, would not able to recommend a \textit{newly-introduced} item, i.e., an item $i$ for which no positive example exists ($r_{ui}=0$ for all users $u$). 
%Similarly, the algorithm would not able to recommend an item to a new user, that is, a user $u$ for which no positive example exists ($r_{ui}=0$ for all $i$). 
%To be able to make recommendations for new items and for new users, additional information has to be leveraged, such as user and item attributes. 
Additional information can be of the form of user and item attributes, such as the affiliation of a user or item with a certain hierarchy or ontology. For example, in the B2B setting, a client-company belongs to a certain industry (automotive, banking, etc.), and in the traditional consumer setting, a movie or a book belongs to one or more genres (biography, fiction, etc.). 

We restrict our attention to the incorporation of a single categorical item attribute, denoted by $A_{i}$, that takes on values in a finite set $\{a_1,...,a_{J}\}$. The extension to several (distinct) item attributes and to user attributes will turn out to be straightforward. 
The item attribute is incorporated into the generative model by assuming that the attribute values $A_{i}$ are generated by the co-cluster affiliations, similarly as the positive examples are generated by the co-cluster affiliations (cf.~Section \ref{seg:genmod}). 
This approach is quite common; for example, in the context of article recommendations, the collaborative topic model \cite{DBLP:conf/kdd/WangB11} assumes that article ratings are generated by latent vectors \emph{and} by topic proportions (i.e., by item attributes). Similarly,
 binary features can be incorporated into the community model by proposing a model that generates both node attributes and edges in the corresponding graph with communities by regarding the community affiliation vectors as the inputs features to a (binary) logistic model \cite{yang_community_2013}. 

%\medskip\noindent\textbf{Generative Model:}
In the same way, we assume that the $A_{i}$ are generated by the co-clusters by regarding the co-cluster affiliation vectors $\vf_u,\vf_i$ as input features to a logistic model. Specifically, %, with associated weight factors. %$w_{0k}, \vw_k \in \reals^K, k = 0,..., J-2$. 
 the probability of $A_{i}$ taking on the value $a_k$ is given by  
\begin{align*}
&\PR{A_{i} = a_{k} | \mF} 
=
\frac{ 
e^{- w_{0k}  - \innerprod{\vw_k}{ \vf_i }  }
}{   
1 + \sum_{\ell=1}^{J-1}
e^{- w_{0\ell}  - \innerprod{\vw_\ell}{ \vf_i } }
}, \quad k = 1,..., J-1, \\
%
&\PR{A_{i} = a_{J} | \mF} 
=
\frac{ 
1
}{   
1 + \sum_{\ell=1}^{J-1}
e^{- w_{0\ell}  - \innerprod{\vw_\ell}{ \vf_i } } 
},
\end{align*}
where $w_{0\ell}, \vw_\ell \in \reals^K, \ell =1,...,J-1$, are the associated weight factors, and $\mF$ contains $\vf_u,\vf_i$ as columns. 
Assuming that attributes are generated independently for each item, the attribute likelihood is given by
\[
\mc L_A 
= \prod_i \PR{A_i | \mF, \mW },
\]
where the product is over all items $i$ that have a feature associated with them, and $\mW$ denotes the set of associated weight factors $w_{0\ell}, \vw_\ell \in \reals^K, \ell =1,...,J-1$. Assuming that the positive examples and the attributes are generated independently based on the community membership, the negative model log likelihood of the overall model is given by $-\log \tilde {\mc L} = -\log \mc L - \mu \log \mc L_A$, where $\mu$ is a parameter that weights the likelihoods. 
To find the factors $\vf_u,\vf_i$ and the weights of the logistic model $w_{0\ell}, \vw_\ell$, we solve---analogously as in \eqref{eq:optprob}---the following optimization problem: 
\begin{align}
\text{minimize } \tilde Q \text { subject to } [\vf_{u}]_c, [\vf_{i}]_c  \geq 0, \forall c,
\label{eq:optprobfeat}
\end{align}
where 
\[
\tilde Q = -\log \mc L - \mu \log \mc L_A + \lambda \sum_i \norm[2]{\vf_i}^2  + \lambda \sum_u \norm[2]{\vf_u}^2.
\]
Here, $\lambda\geq 0$ is a regularization parameter, and minimization is with respect to the factors $\vf_{u}, \vf_i$ and the weights $w_{0\ell}, \vw_\ell$. 

Similarly as before, one can use a cyclic block coordinate descent approach to minimize \eqref{eq:optprobfeat}. Specifically, we iteratively update first $\vf_u$, then  $\vf_i$, both via projected gradient descent, and finally the weights $w_{0\ell}, \vw_\ell$, with gradient descent. 
We finally note that this variant of OCuLaR is very efficient; specifically, the complexity of updating all factors and weights is 
$
O(|\{(i,u)\colon r_{ui}=1\}|  K  +  J K N),
$ 
where $N$ is the number of items. 



==> Overlapping CoClusters (2017)/gpu.tex <==
\section{Using Massively Parallel Processors}
\label{sec:gpu}

The OCuLaR algorithm can be dramatically accelerated by exploiting its inherent parallelism. In fact, one can easily map and implement the costly training phase onto a graphics processing unit (GPU). This results in two benefits:

\begin{itemize}
    \item Leverage the \textbf{reduction in training time} to train the model and produce recommendations in significantly reduced time. For the real industrial dataset used in our experiments, both training of the model and generation of recommendations can be completed in mere seconds when using a GPU.
    \item Perform a more \textbf{fine-grained grid search} over the algorithm's hyper-parameters to obtain a higher precision/recall. OCuLaR requires the learning of $K$ (number of co-clusters) and $\lambda$ by using a cross-validated grid search. This phase can be costly, so in practice one can only search across a certain range of values and keep the pair that results in the best performance under the desirable accuracy metric. Achieving very fast learning using GPUs essentially allows the methodology to examine a broader range of hyper-parameter value pairs that help improve the overall accuracy.
\end{itemize}
 In order to achieve the potential acceleration offered by GPU devices, communication of large amounts of data between the host and the device must be avoided, especially during iterative computations. Furthermore, arithmetic computations must be carefully designed to optimally make use of the underlying computational architecture and memory hierarchy. Below, we describe in more detail how OCuLaR can be mapped onto an efficient GPU implementation.

\subsection{GPU implementation}

We begin by describing how data moves between the host and the GPU during the training of the OCuLaR algorithm. Firstly, the entire training data (in a sparse format) is copied from the host memory into the GPU main memory along with a set of initial values for the $\vf_i$ and $\vf_u$ vectors. The iterative training algorithm described in Section \ref{sec:impdet} is then performed by launching a sequence of kernel functions. Throughout the training, all data remains on the GPU and communication back and forth between the host and the device is limited to a small amount of control logic. Once a predetermined set of iterations has been executed, the learned values of the $\vf_i$ and $\vf_u$ are copied back from the GPU to the host memory and the training is completed. 

%\vspace{-\baselineskip}
\begin{figure}[!h]
\centering
\includegraphics[width=\columnwidth]{figures/gpu_arch.png}
\caption{Computation of the gradient vector is performed by a large number of thread blocks that are executed on the streaming multiprocessors of the GPU}
\label{fig:gpu_arch}
\end{figure}


The arithmetic computations that comprise the training are split into a number of separate kernel functions. As an illustration, we provide a detailed description of how the kernel that computes the gradient vectors for all items is structured to efficiently use the underlying hardware. We begin by noting that equation (\ref{eq:origgrad}) can be expressed:
\begin{eqnarray}
\nabla Q( \vf_i ) 
&=& \sum_{u}\vf_u + 2 \lambda \vf_i - 
\sum_{u\colon r_{ui} = 1}  \vf_u \left(1 -e^{-  \innerprod{\vf_u}{ \vf_i} }\right)^{-1}\nonumber\\
&=& C + 2 \lambda \vf_i - \sum_{u\colon r_{ui} = 1}  \vf_u \alpha(\innerprod{\vf_u}{ \vf_i}),
\label{eq:gpugrad}
\end{eqnarray}
where $C$ is a constant independent of the item index. As in the reference CPU-only implementation, an initial computation is performed to calculate the sum of all $\vf_u$ vectors and the gradient vectors are initialized in GPU memory as $C+2\lambda\vf_i$. A kernel function is then called which launches a thread block for every positive rating in the training data. Since this number is typically very large, this mapping is well suited to the massively parallel GPU architecture in which a number of streaming multiprocessors are capable of executing multiple thread blocks concurrently. 

We will now describe the computation performed by a single thread block in more detail, making reference to Figure \ref{fig:gpu_arch}. The thread block first fetches the corresponding $\vf_i$ vector and $\vf_u$ vector from GPU main memory and computes the inner product between the two. Following the approach of \cite[p. 76]{sanders2010cuda}, an individual thread within the block handles computation of only part of the inner product. The memory access patterns are carefully arranged so that threads that are executed concurrently (as a "warp") access contiguous regions of memory, allowing reads to be effectively coalesced. The partial results are then stored in high-speed shared memory and a reduction is performed to obtain the final value of the inner product ($P$). A single thread within the block then computes the scalar $\alpha$. Finally, the thread block multiplies this scalar by the $\vf_u$ vector and updates the corresponding item gradient in GPU main memory using atomic operations. In this manner, the sum in equation~\eqref{eq:gpugrad} is computed entirely asynchronously for all items. Once all the thread blocks have finished execution, the correct value of the gradient vectors exist in GPU main memory and the training can proceed. The other essential computations, such as the evaluation of the likelihood function are mapped to the GPU in a similar fashion.

\noindent\textbf{Memory:} The memory footprint of the GPU-based OCuLaR implementation scales as:
\begin{equation}
O\left(\max
\left(|\{(u,i):r_{ui}=1\}|,n_uK,n_iK\right)\right),\nonumber
\end{equation}
where $n_u$ and $n_i$ are the number of users and the number of items respectively. This property allows for training on very large datasets despite the relatively limited memory capacity of modern GPU devices. For example, around 2.7GB of GPU memory is required to train on the Netflix dataset (assuming $K=200$) and thus the problem easily fits within the main memory of an inexpensive GPU (typically up to 12GB). In contrast, a previous attempt to implement an alternating-least-square based matrix factorization approach on GPUs determined that the memory requirements for the same dataset exceeded 12GB (for the equivalent of K=100) \cite{tan2016faster}.  

==> extra_information.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\vspace{-2\baselineskip}
\section{Adding extra information}
\label{sec:incorpatt}

While the focus of this paper is on generating recommendations based on positive examples only, e.g., on the purchase history of clients, we explain briefly  how to incorporate additional information in the OCuLaR algorithm. 
This is important for addressing the cold-start problem, i.e., for making recommendations to users that have no purchase history, or for recommending items that have not been purchased. In addition, it can also improve the recommendation performance for users/items for which positive examples exist. 
%An astute reader would have noticed that the algorithm, as previously described, would not able to recommend a \textit{newly-introduced} item, i.e., an item $i$ for which no positive example exists ($r_{ui}=0$ for all users $u$). 
%Similarly, the algorithm would not able to recommend an item to a new user, that is, a user $u$ for which no positive example exists ($r_{ui}=0$ for all $i$). 
%To be able to make recommendations for new items and for new users, additional information has to be leveraged, such as user and item attributes. 
Additional information can be of the form of user and item attributes, such as the affiliation of a user or item with a certain hierarchy or ontology. For example, in the B2B setting, a client-company belongs to a certain industry (automotive, banking, etc.), and in the traditional consumer setting, a movie or a book belongs to one or more genres (biography, fiction, etc.). 

We restrict our attention to the incorporation of a single categorical item attribute, denoted by $A_{i}$, that takes on values in a finite set $\{a_1,...,a_{J}\}$. The extension to several (distinct) item attributes and to user attributes will turn out to be straightforward. 
The item attribute is incorporated into the generative model by assuming that the attribute values $A_{i}$ are generated by the co-cluster affiliations, similarly as the positive examples are generated by the co-cluster affiliations (cf.~Section \ref{seg:genmod}). 
This approach is quite common; for example, in the context of article recommendations, the collaborative topic model \cite{DBLP:conf/kdd/WangB11} assumes that article ratings are generated by latent vectors \emph{and} by topic proportions (i.e., by item attributes). Similarly,
 binary features can be incorporated into the community model by proposing a model that generates both node attributes and edges in the corresponding graph with communities by regarding the community affiliation vectors as the inputs features to a (binary) logistic model \cite{yang_community_2013}. 

%\medskip\noindent\textbf{Generative Model:}
In the same way, we assume that the $A_{i}$ are generated by the co-clusters by regarding the co-cluster affiliation vectors $\vf_u,\vf_i$ as input features to a logistic model. Specifically, %, with associated weight factors. %$w_{0k}, \vw_k \in \reals^K, k = 0,..., J-2$. 
 the probability of $A_{i}$ taking on the value $a_k$ is given by  
\begin{align*}
&\PR{A_{i} = a_{k} | \mF} 
=
\frac{ 
e^{- w_{0k}  - \innerprod{\vw_k}{ \vf_i }  }
}{   
1 + \sum_{\ell=1}^{J-1}
e^{- w_{0\ell}  - \innerprod{\vw_\ell}{ \vf_i } }
}, \quad k = 1,..., J-1, \\
%
&\PR{A_{i} = a_{J} | \mF} 
=
\frac{ 
1
}{   
1 + \sum_{\ell=1}^{J-1}
e^{- w_{0\ell}  - \innerprod{\vw_\ell}{ \vf_i } } 
},
\end{align*}
where $w_{0\ell}, \vw_\ell \in \reals^K, \ell =1,...,J-1$, are the associated weight factors, and $\mF$ contains $\vf_u,\vf_i$ as columns. 
Assuming that attributes are generated independently for each item, the attribute likelihood is given by
\[
\mc L_A 
= \prod_i \PR{A_i | \mF, \mW },
\]
where the product is over all items $i$ that have a feature associated with them, and $\mW$ denotes the set of associated weight factors $w_{0\ell}, \vw_\ell \in \reals^K, \ell =1,...,J-1$. Assuming that the positive examples and the attributes are generated independently based on the community membership, the negative model log likelihood of the overall model is given by $-\log \tilde {\mc L} = -\log \mc L - \mu \log \mc L_A$, where $\mu$ is a parameter that weights the likelihoods. 
To find the factors $\vf_u,\vf_i$ and the weights of the logistic model $w_{0\ell}, \vw_\ell$, we solve---analogously as in \eqref{eq:optprob}---the following optimization problem: 
\begin{align}
\text{minimize } \tilde Q \text { subject to } [\vf_{u}]_c, [\vf_{i}]_c  \geq 0, \forall c,
\label{eq:optprobfeat}
\end{align}
where 
\[
\tilde Q = -\log \mc L - \mu \log \mc L_A + \lambda \sum_i \norm[2]{\vf_i}^2  + \lambda \sum_u \norm[2]{\vf_u}^2.
\]
Here, $\lambda\geq 0$ is a regularization parameter, and minimization is with respect to the factors $\vf_{u}, \vf_i$ and the weights $w_{0\ell}, \vw_\ell$. 

Similarly as before, one can use a cyclic block coordinate descent approach to minimize \eqref{eq:optprobfeat}. Specifically, we iteratively update first $\vf_u$, then  $\vf_i$, both via projected gradient descent, and finally the weights $w_{0\ell}, \vw_\ell$, with gradient descent. 
We finally note that this variant of OCuLaR is very efficient; specifically, the complexity of updating all factors and weights is 
$
O(|\{(i,u)\colon r_{ui}=1\}|  K  +  J K N),
$ 
where $N$ is the number of items. 


